Finite-size reversal of a multiparticle correction to local spin spectra in a flux-disordered Kitaev honeycomb model

A spin flip in the Kitaev honeycomb model changes the flux background and therefore the Hamiltonian seen by the matter fermions. Can a one-particle approximation with the correct total spin intensity nevertheless misestimate the depth of a depression in the local spin spectrum? We test this question in a frozen, flux-disordered ensemble by retaining the actual one-particle transition energies and relative spectral weights after the spin flip, then rescaling those weights to match the full intensity. We measure the depression by subtracting the central intensity from the average at two flanking frequencies. For spin-created states with odd final quasiparticle number and nonzero one-particle weight, restoring multiparticle weight shallows the depression on 24 sites and deepens it on both 1,536-site shapes and the 3,456- and 6,144-site tori, as judged by the median paired correction at each of two energy resolutions. For these states, the one-particle approximation overestimates the mean dip depth by about 16-18% on 24 sites and underestimates it by 33-56% in the 6,144-site sample. Extrapolating from 24 sites would therefore give the wrong sign for this correction on those four larger tori under the same disorder prescription.

==> tables/absolute_rows.tex <==
\def\AbsoluteRows{%
24, all & 0.05 & $[8.173,8.174]$ & $[7.697,7.698]$ & $[2.831,2.832]$ & $[2.837,2.838]$ & $[4.864,4.865]$ & $[4.799,4.800]$ \\
24, odd & 0.05 & $[9.769,9.770]$ & $[8.759,8.760]$ & $[2.996,2.997]$ & $[3.009,3.010]$ & $[4.847,4.848]$ & $[4.711,4.712]$ \\
96 & 0.05 & $[6.495,6.496]$ & $[6.381,6.424]$ & $[2.675,2.676]$ & $[2.815,2.861]$ & $[4.631,4.632]$ & $[5.283,5.328]$ \\
384 & 0.05 & $[5.660,5.661]$ & $[6.141,6.186]$ & $[3.047,3.048]$ & $[3.318,3.365]$ & $[3.435,3.436]$ & $[4.680,4.733]$ \\
1536 & 0.05 & $[5.850,5.851]$ & $[6.585,6.637]$ & $[2.873,2.874]$ & $[3.233,3.284]$ & $[3.317,3.318]$ & $[5.066,5.123]$ \\
3456 & 0.05 & $[4.424,4.425]$ & $[5.588,5.646]$ & $[2.554,2.555]$ & $[3.165,3.221]$ & $[2.645,2.646]$ & $[4.864,4.925]$ \\
6144 & 0.05 & $[4.974,4.975]$ & $[5.969,6.033]$ & $[3.169,3.171]$ & $[3.618,3.681]$ & $[3.163,3.165]$ & $[4.895,4.964]$ \\
1536 rect. & 0.05 & $[5.349,5.350]$ & $[6.160,6.213]$ & $[2.384,2.385]$ & $[2.767,2.820]$ & $[3.277,3.278]$ & $[4.904,4.962]$ \\
\midrule
24, all & 0.10 & $[15.632,15.633]$ & $[14.732,14.733]$ & $[6.352,6.353]$ & $[6.343,6.344]$ & $[9.623,9.624]$ & $[9.501,9.502]$ \\
24, odd & 0.10 & $[18.412,18.413]$ & $[16.502,16.503]$ & $[6.965,6.966]$ & $[6.947,6.948]$ & $[9.855,9.856]$ & $[9.596,9.597]$ \\
96 & 0.10 & $[13.102,13.103]$ & $[12.677,12.720]$ & $[5.815,5.816]$ & $[6.064,6.112]$ & $[9.179,9.180]$ & $[10.417,10.465]$ \\
384 & 0.10 & $[11.966,11.967]$ & $[12.541,12.590]$ & $[6.150,6.151]$ & $[6.787,6.839]$ & $[6.937,6.938]$ & $[9.323,9.381]$ \\
1536 & 0.10 & $[11.848,11.849]$ & $[12.926,12.983]$ & $[5.621,5.622]$ & $[6.412,6.468]$ & $[6.685,6.686]$ & $[10.006,10.069]$ \\
3456 & 0.10 & $[9.894,9.895]$ & $[11.617,11.679]$ & $[5.231,5.232]$ & $[6.491,6.552]$ & $[5.324,5.325]$ & $[9.505,9.573]$ \\
6144 & 0.10 & $[10.791,10.792]$ & $[12.259,12.328]$ & $[6.137,6.138]$ & $[7.177,7.246]$ & $[6.250,6.252]$ & $[9.520,9.597]$ \\
1536 rect. & 0.10 & $[11.478,11.479]$ & $[12.598,12.655]$ & $[5.046,5.047]$ & $[5.917,5.974]$ & $[6.709,6.710]$ & $[9.804,9.867]$ \\
}


==> tables/cohort_mean_rows.tex <==
\def\CohortRows{%
% Printed Table S6 inputs; exact factor 170/320; outward-rounded endpoints.
% Units: 10^{-3} absolute spin intensity. Realized-cohort numerical bounds.
$0.05$ & $[-0.9767,-0.8567]$ & $[-0.5189,-0.4551]$ \\
$0.10$ & $[-1.3953,-1.2656]$ & $[-0.7413,-0.6723]$ \\
}


==> tables/median_rows.tex <==
\def\MedianRows{%
24 (exact) & 0.05 & --- & $[-0.129,-0.128]$ & $[-0.096,-0.094]$ & $[-0.120,-0.119]$ & $[1.407,1.409]$ \\
96 & 0.05 & 164 & $[0.178,2.089]$ & $[0.066,1.363]$ & $[-0.276,1.075]$ & $[-2.428,1.694]$ \\
384 & 0.05 & 156 & $[0.297,3.084]$ & $[0.262,2.215]$ & $[0.193,1.960]$ & $[-4.517,0.239]$ \\
1536 & 0.05 & 175 & $[0.521,2.479]$ & $[0.394,1.662]$ & $[0.276,1.712]$ & $[-5.688,-1.164]$ \\
3456 & 0.05 & 177 & $[0.586,2.604]$ & $[0.509,2.016]$ & $[0.653,1.781]$ & $[-7.717,-1.784]$ \\
6144 & 0.05 & 170 & $[0.576,3.186]$ & $[0.652,2.330]$ & $[0.671,2.080]$ & $[-5.744,-0.943]$ \\
1536 rect. & 0.05 & 135 & $[0.461,2.440]$ & $[0.430,2.272]$ & $[0.405,2.250]$ & $[-5.335,-0.744]$ \\
\midrule
24 (exact) & 0.10 & --- & $[-0.525,-0.524]$ & $[-0.392,-0.391]$ & $[-0.490,-0.489]$ & $[3.170,3.171]$ \\
96 & 0.10 & 164 & $[0.070,3.246]$ & $[-0.164,2.385]$ & $[-1.134,1.934]$ & $[-4.347,3.091]$ \\
384 & 0.10 & 156 & $[0.616,5.704]$ & $[0.529,4.278]$ & $[0.467,3.860]$ & $[-7.889,-0.234]$ \\
1536 & 0.10 & 175 & $[1.092,4.941]$ & $[0.752,3.600]$ & $[0.521,3.987]$ & $[-9.502,-2.116]$ \\
3456 & 0.10 & 177 & $[1.475,5.403]$ & $[1.568,4.188]$ & $[1.815,4.762]$ & $[-12.873,-2.945]$ \\
6144 & 0.10 & 170 & $[1.780,6.246]$ & $[1.529,4.801]$ & $[1.513,4.599]$ & $[-9.095,-1.015]$ \\
1536 rect. & 0.10 & 135 & $[0.979,4.675]$ & $[1.194,4.845]$ & $[1.047,4.539]$ & $[-8.977,-1.314]$ \\
}


==> tables/normalization_rows.tex <==
\def\NormalizationRows{%
24 & 0.05 & 3892 & $[0.5861,0.5862]$ & $[0.5696,0.5698]$ \\
24 & 0.10 & 3892 & $[1.0663,1.0665]$ & $[0.9925,0.9926]$ \\
6144 & 0.05 & 170 & $[-0.9767,-0.8567]$ & $[-1.2502,-1.1292]$ \\
6144 & 0.10 & 170 & $[-1.3953,-1.2656]$ & $[-1.7007,-1.5704]$ \\
}


==> tables/odd_depth_fit_rows.tex <==
\def\FittedDepthRows{%
Four & $1/L$ & $[-5.042,-4.194]$ & $[-6.613,-2.606]$ & $[-7.598,-6.685]$ & $[-10.220,-4.049]$ \\
Four & $1/L^2$ & $[-4.370,-3.805]$ & $[-5.424,-2.739]$ & $[-6.604,-5.997]$ & $[-8.356,-4.225]$ \\
Three & $1/L$ & $[-5.010,-3.490]$ & $[-8.137,-0.379]$ & $[-6.682,-5.050]$ & $[-11.889,0.179]$ \\
Three & $1/L^2$ & $[-4.536,-3.661]$ & $[-6.357,-1.823]$ & $[-6.449,-5.508]$ & $[-9.495,-2.437]$ \\
}


==> tables/odd_depth_mean_rows.tex <==
\def\MeanDepthRows{%
96 & $[-0.686,-0.333]$ & $[-1.882,0.901]$ & $[-0.813,-0.445]$ & $[-2.751,1.572]$ \\
384 & $[-2.559,-2.185]$ & $[-3.959,-0.821]$ & $[-3.581,-3.174]$ & $[-5.879,-0.885]$ \\
1536 & $[-3.739,-3.336]$ & $[-5.026,-2.037]$ & $[-5.856,-5.428]$ & $[-8.003,-3.267]$ \\
3456 & $[-4.545,-4.114]$ & $[-6.117,-2.424]$ & $[-7.006,-6.542]$ & $[-9.672,-3.722]$ \\
6144 & $[-3.907,-3.427]$ & $[-5.504,-1.824]$ & $[-5.582,-5.062]$ & $[-8.217,-2.390]$ \\
1536 rect. & $[-3.554,-3.145]$ & $[-5.064,-1.635]$ & $[-5.165,-4.732]$ & $[-7.662,-2.208]$ \\
}


==> tables/stability_rows.tex <==
\def\StabilityRows{%
$3456-1536$ & $[-1.153,1.621]$ & $[-6.552,3.903]$ & $[-2.031,3.436]$ & $[-10.757,6.557]$ \\
$6144-3456$ & $[-1.363,1.821]$ & $[-3.959,6.773]$ & $[-2.658,3.233]$ & $[-6.150,11.857]$ \\
$6144-1536$ & $[-1.010,1.936]$ & $[-4.579,4.744]$ & $[-2.071,4.049]$ & $[-6.979,8.487]$ \\
$1536$, rectangle $-$ tilted & $[-1.232,1.878]$ & $[-4.170,4.944]$ & $[-2.405,4.093]$ & $[-6.861,8.188]$ \\
}

